Shape or Texture: Understanding Discriminative Features in CNNs

Contrasting the previous evidence that neurons in the later layers of a Convolutional Neural Network (CNN) respond to complex object shapes, recent studies have shown that CNNs actually exhibit a `texture bias': given an image with both texture and shape cues (e.g., a stylized image), a CNN is biased towards predicting the category corresponding to the texture. However, these previous studies conduct experiments on the final classification output of the network, and fail to robustly evaluate the bias contained (i) in the latent representations, and (ii) on a per-pixel level. In this paper, we design a series of experiments that overcome these issues. We do this with the goal of better understanding what type of shape information contained in the network is discriminative, where shape information is encoded, as well as when the network learns about object shape during training. We show that a network learns the majority of overall shape information at the first few epochs of training and that this information is largely encoded in the last few layers of a CNN. Finally, we show that the encoding of shape does not imply the encoding of localized per-pixel semantic information. The experimental results and findings provide a more accurate understanding of the behaviour of current CNNs, thus helping to inform future design choices.

==> exp.tex <==
\section{Do CNNs Spend More Learning Capacity on Shape or Texture?}\label{sec:docnns}
With the goal of revealing the characteristics of \textit{where}, \textit{when}, and \textit{how much} shape information is encoded in CNNs, we first aim to quantify the number of dimensions which encode shape in a CNN's latent representation. This analysis on the latent representations will allow us to determine \textit{where} the network spends learning capacity on shape, while other methods that focus solely on the network outputs have difficulty measuring the difference in shape information between convolutional layers.
%Additionally, it can reveal how strong the correlation is between the amount of shape information encoded in a CNN, and the number of dimensions used to encode this information.
 
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure} [t]
\centering
  \begin{center}
  \resizebox{0.99\textwidth}{!}{ 
  %\vspace{-0.55cm}
      \includegraphics[width=0.99\textwidth]{figures/shape4.pdf}}
  \end{center}
  \vspace{-0.3cm}
  \caption{\textcolor{black}{Illustration of the techniques used to quantify shape in this paper}. \textbf{(A)} Estimating the dimensionality of semantic concepts in latent representations: We stylize each image with five textures to generate image pairs which share the semantic concepts \textit{shape} (right pair) and \textit{texture} (left pair). We feed these image pairs (shown is \textit{shape}) to an encoder, $E(\cdot)$, and calculate the mutual information between the two latent representations, $z^a$ and $z^b$, to estimate the dimensionality, $|z_{\text{shape}}|$. \textbf{(B)} We quantify the shape information encoded in a convolutional neural network by freezing the weights, and then training a small read-out module (i.e., three 3$\times$3 convolutional layers) on the latent representation to predict either a binary or semantic segmentation map.}
  \label{fig:stylize}
  %\vspace{-0.45cm}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Estimating shape and texture dimensionality}\label{sec:dimension}
\newcommand{\covariance}[1]{\text{Cov}\bigl(#1\bigr)}
\newcommand{\variance}[1]{\text{Var}(#1)}
\newcommand{\MI}{\operatorname{MI}}

Previous works~\citep{bau2017network,esser2020disentangling} proposed various
mechanisms to reveal the semantic concepts encoded in latent representations of
CNNs. To quantify the amount of texture and shape information, we
follow the approach of \citep{esser2020disentangling}, where the number of
neurons that represent a certain semantic concept is estimated.
%After a brief
%description of this estimate, we evaluate how consistent it can predict the
%relative importance of concepts by comparing its results to those of an
%alternative estimate given by \citep{bau2017network}.
Given a pretrained CNN encoder, $E(I)=z$, where $z$ is a latent representation,
we aim to estimate the dimensionality of the semantic concepts shape and
texture within $z$.
The main idea is that the mutual information between image pairs, $I^a$ and $I^b$,
which are similar in a semantic concept, will be preserved in a neuron $z_i$
only if the neuron encodes that specific semantic concept. Hence, the mutual
information between the corresponding neuron pairs, $z_i^a = E(I^a)$ and $z_i^b =
E(I^b)$, can be used to quantify the degree to which a semantic concept is
represented by the neuron.
A simple and efficient estimate for their mutual information $\MI(z_i^a, z_i^b)$
can be obtained based on the correlation coefficient $\rho_i$. Indeed, under the assumption that the marginal distribution of the neuron $z_i$ is
Gaussian, the correlation coefficient $\rho_i$ provides a lower bound on the
true mutual information through the following relationship which becomes tight for jointly Gaussian $z_i^a, z_i^b$~\citep{kraskov2004estimating,foster2011lower}.
\begin{equation}
  \MI(z_i^a, z_i^b) \ge -\frac{1}{2} \log (1 - \rho_i^2), \quad \text{where  }
  \rho_i = \frac{\covariance{z_i^a, z_i^b}}{
        \sqrt{\variance{z_i^a} \;\variance{z_i^b}}}.
  \label{eq:correlation}
\end{equation}

% Indeed, under the assumption that the marginal distribution of the neuron $z_i$ is
% Gaussian, the correlation coefficient $\rho_i$ provides a lower bound on the
% true mutual information through the relationship
% \begin{equation}
%   \MI(z_i^a, z_i^b) \ge -\frac{1}{2} \log (1 - \rho_i^2),
% \end{equation}


To quantify how well a concept $k$ is represented in terms of the number of
neurons $\vert z_k \vert$ that encode the concept, we compute a score for each concept and
the relative number of neurons is determined with a softmax over these scores and
a baseline score.
%Following \citep{esser2020disentangling},
The latter is given
by the number of neurons $\vert z \vert$, and shape and texture scores are given by the sum of
their respective correlation coefficients $\rho_i^{\text{shape}}$ and
$\rho_i^{\text{texture}}$, which are computed according to Eq.~\ref{eq:correlation}
with statistics taken over image pairs that are similar in shape and texture,
respectively. Note that $k\in\{1,2\}$ in our case, and the remaining dimensions not captured in any of the two semantic factors are allocated to the \textit{residual} semantic factor, which by definition captures all other variability in the latent representation, $z$. 
%Examples of these image pairs are shown in Fig.~\ref{fig:stylize}
%and their construction is described next.
% full formula, here if space, supplementary otherwise
%\begin{equation}
%  \vert z_k \vert = \left\lfloor \frac{\exp{\sum_i \rho_i^k}}{\exp{\sum_i
%  \rho_i^\text{shape}}+\exp{\sum_i \rho_i^\text{texture}}+\exp{\vert z\vert}}
%  \right\rfloor \vert z \vert
%  \quad k \in \{\text{shape}, \text{texture}\}
%\end{equation}

%%%%%%%%%%%%%%

% \begin{table} [t]
% \vspace{-0.2cm}
% 	\centering
% 	\begin{minipage}{0.64\linewidth}
% 	      %\vspace{0.7cm}
%           \centering
%          \resizebox{1.0\textwidth}{!}{
%           \includegraphics[width=0.43\textwidth]{figures/shape2.pdf} 
%     }
%   \vspace{-0.5cm}
%   \captionof{figure}{Sample generation of validation examples for different semantic concepts.}
%   \label{fig:dim_concept}
% 	\end{minipage} \hfill
% 	\begin{minipage}{0.34\linewidth}
% 	\caption{Dimensionality estimation of factors $z_K$ representing different semantic concepts for different BagNet variants.} %and evaluated on two different GT patterns
% 	\centering
% 	\vspace{-0.25cm}
% 	\def\arraystretch{1.1}
% 	\setlength\tabcolsep{3.2pt}
% 		\resizebox{0.85\textwidth}{!}{
% 			\begin{tabular}{r|cc }

% 	\specialrule{1.2pt}{1pt}{1pt}
	 
% 	 \multirow{2}{*}{\hspace{0.01cm} \rotatebox{0}{Model}}  & \multicolumn{2}{c}{Factor $z_K$}\\
	 
% 	 \cline{2-3}
% 	   &  Shape & Texture\\
% 	 \specialrule{1.2pt}{1pt}{1pt}
	 
% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{ResNet50}}  &
	  
% 	  \textbf{349} & 692 \\
	 
% 	  \hline

% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{BagNet33}}  &
        
% 	  284 & 825\\
	  
% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{BagNet17}}  &
	  
% 	  278 & 839 \\
	  
% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{BagNet9}}  &
	  
% 	  276 & \textbf{841} \\
% 	\specialrule{1.2pt}{1pt}{1pt}

% 	\end{tabular}
% \label{tab:bagnet_dim}
% 			}
% 			\end{minipage}
	    
% 	\vspace{-0.3cm}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure} [t]
%   \begin{center}
%   \resizebox{0.6\textwidth}{!}{ 
%   %\vspace{-0.55cm}
%       \includegraphics[width=0.50\textwidth]{figures/shape2.pdf}}
%   \end{center}
%   \vspace{-0.35cm}
%   \caption{Sample generation of validation examples for different semantic concepts.}
%   \label{fig:stylize}
%   %\vspace{-0.45cm}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Stylized PASCAL VOC 2012 Dataset}\label{sec:stylized_voc}
%The dimensionality estimation relies on image pairs which are similar in shape
%and texture.

%To obtain such pairs,
\noindent \textbf{Stylized PASCAL VOC 2012 Dataset.} 
Our goal is to estimate the dimensionality of two semantic concepts: (i) \textit{shape} and (ii) \textit{texture}, and analyze pixel-wise shape information. Therefore we must generate a dataset that we can sample image pairs which share the semantic factors shape or texture, and have per-pixel object annotations.
To accomplish this goal, we create the \textit{Stylized PASCAL VOC
2012} (SVOC) dataset. Similar to SIN, we use the AdaIN style transfer algorithm~\citep{huang2017arbitrary} to generate
stylized images from the PASCAL VOC 2012 dataset~\citep{PASCALVOC} with the
same settings and hyperparameters as in the original
paper~\citep{huang2017arbitrary}. We choose five random textures from the Describable Textures
Dataset~\citep{cimpoi2014describing} as the styles and we stylize every PASCAL
VOC image with all five of these textures. For a fair comparison with models
trained on ImageNet variants, we take only the images from PASCAL VOC which
contain a single object. With the SVOC dataset, we can now sample image pairs
which are similar in \textit{texture}, by using two images from
different categories but stylized with the same texture
(Fig.~\ref{fig:stylize}(A) left), or \textit{shape}, by using the same image stylized with two different textures (Fig.~\ref{fig:stylize}(A) right).


% \textit{shape}, by using the same image stylized with two different
% textures (Fig.~\ref{fig:stylize}(A) right), or texture, by using two images from
% different categories but stylized with the same texture
% (Fig.~\ref{fig:stylize}(A) left).
%which share one of two semantic concepts (see Fig.~\ref{fig:stylize}). For a
%given SVOC image, we randomly select a semantic factor: shape or texture. If
%shape is drawn, then we sample the \textit{same image} but with a
%\textit{different texture} (see Fig.~\ref{fig:stylize}, top). Alternatively, if
%texture is sampled, we select a random image from a \textit{different category}
%but with the \textit{same texture} (see Fig.~\ref{fig:stylize}, bottom).
% TODO do we need to introduce the the residual?
%The
%remaining dimensions not captured in either the \textit{shape} or
%\textit{texture} is allocated to the \textit{residual} semantic factor, which
%by definition captures all other variability in latent representation, $z$.
% TODO do we need this clarification?
%Note that `object shape' in our experiments refers to the \textit{convex
%outline of an object}. 

%%%%%%%%%%%%%%%%
\begin{table}[t]
\vspace{-0.2cm}
\def\arraystretch{1.15}
\centering
\caption{\textbf{Dimensionality estimation} of semantic factors $|z_k|$ for the stage-5 latent representation. Note that the total dimension of the latent representation, $|z|$, is 2048 for all networks, and that the remaining dimensions are allocated to the `residual' factor. (a) ResNet50 compared with BagNets. BagNets have more neurons which encode \textit{texture} than \textit{shape} due to their restricted receptive field. (b) Networks with varying levels of shape bias. The number of neurons which encode shape correlates with shape bias. (c) Deeper networks contain more \textit{shape} encoding neurons.}
%  IN: trained on ImageNet, SIN: trained on Stylized ImageNet, ((SIN+IN)$\rightarrow$IN): trained on SIN and IN, and then fine-tuned on IN.
     \vspace{-0.2cm}
\resizebox{0.90\textwidth}{!}{
	\begin{tabular}{c|cc }

	\specialrule{1.2pt}{1pt}{1pt}
	 
	 \multirow{2}{*}{\hspace{0.01cm} \rotatebox{0}{Model}}  & \multicolumn{2}{c}{Factor $|z_k|$}\\
	 
	 \cline{2-3}
	   &  Shape & Texture\\
	 \specialrule{1.2pt}{1pt}{1pt}
	 
	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{ResNet50}}  &
	  
	  \textbf{349} & 692 \\
	 
	  \hline

	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{BagNet33}}  &
        
	  284 & 825\\
	  
	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{BagNet17}}  &
	  
	  278 & 839 \\
	  
	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{BagNet9}}  &
	  
	  276 & \textbf{841} \\
	\specialrule{1.2pt}{1pt}{1pt}

	\end{tabular}

	\hspace{0.2cm}
	

		\begin{tabular}{c|cc }

	\specialrule{1.2pt}{1pt}{1pt}
	 
	 \multirow{2}{*}{\rotatebox{0}{Training Data}}  & \multicolumn{2}{c}{Factor $|z_k|$}\\
	 
	 \cline{2-3}
	   &  Shape & Texture\\
	 \specialrule{1.2pt}{1pt}{1pt}
	 
	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{IN}}  &
	  

	  349 & \textbf{692} \\
	  
	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{SIN}}  &
	  

	  \textbf{536} & 477 \\
	  

	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{(SIN+IN)$\rightarrow$IN}}  &
	  

	  376 & 640\\
	 
	\specialrule{1.2pt}{1pt}{1pt}

	\end{tabular}
		\hspace{0.2cm}
	\begin{tabular}{c|cc }

	\specialrule{1.2pt}{1pt}{1pt}
	 
	 \multirow{2}{*}{ \rotatebox{0}{Model}}  & \multicolumn{2}{c}{Factor $|z_k|$}\\
	 
	 \cline{2-3}
	   &  Shape & Texture\\
	 \specialrule{1.2pt}{1pt}{1pt}
	 
% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{ResNet18}}  &
	  

% 	  18.4\% & \textbf{31.2\%} \\
	  
% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{ResNet34}}  &
	  

% 	  18.0\% & \textbf{31.8\%} \\
	  

	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{ResNet50}}  &
	  

	  349 & \textbf{692}\\
	  
	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{ResNet101}}  &
	  

	  365 & 667\\
	
	\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{ResNet152}}  &
	  

	  \textbf{371} & 661\\
	 
	\specialrule{1.2pt}{1pt}{1pt}

	\end{tabular}
	
	}
	
	\label{tab:table1}
	\vspace{-0.45cm}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.15cm}
\subsection{Results}\label{sec:dim_res}
% \vspace{-0.2cm}
We now evaluate the efficacy of the dimensionality estimation method by comparing two networks which
differ significantly in their ability to encode shape information. The first is
a standard ResNet50 architecture and the second is the
recently proposed BagNet~\citep{brendel2019approximating}. BagNets are a modified version of ResNet50 that restrict the height and width of the effective receptive field of the CNN to be a fixed maximum, 
i.e., either 9, 17, or 33 pixels. This patch-based construction precludes
BagNets from classifying images based on extended shape cues. The
results of this comparison are presented in Table~\ref{tab:table1}(a) where
both the ResNet50 and the BagNet variants are trained on
IN. Note that `Stage' refers to a residual block in a ResNet (i.e., there are five stages in ResNet) and all experiments in Table~\ref{tab:table1} use the stage-5 features. As expected, BagNets have more neurons encoding texture than the ResNet50 and there is a clear
correlation between the receptive field of the network and the amount of shape
encoded. As the receptive field decreases, the number of neurons encoding
texture increases even further, while the number of neurons encoding shape decreases.

We now examine whether the `shape bias' metric~\citep{geirhos2018imagenet} correlates with the number of shape encoding neurons. Table~\ref{tab:table1}(b) compares the estimated dimensionality of a ResNet50 trained on ImageNet against networks which are biased towards shape using two different training strategies: (i) training solely on SIN and (ii) training on SIN and IN simultaneously followed by fine-tuning on IN (denoted as (SIN+IN)$\rightarrow$IN, which achieves the best accuracy on ImageNet top-1\% out of the three variations~\citep{geirhos2018imagenet}). ResNet50 trained on IN has far more neurons dedicated to encoding texture than shape. There is a large difference when training a ResNet solely on SIN, where it has less neurons which encode texture than shape. When trained and fine-tuned on (SIN+IN) and IN, respectively, there is an increase in the number of neurons which encode shape compared to IN. 

We consider if there is any pattern in the number of neurons encoding shape or texture as the network depth increases. We compare ResNets with 50, 101, and 152 layers, as they share the underlying layer structure and dimensionality in the final latent representation. As can be seen in Table~\ref{tab:table1}(c), networks have more shape and less texture neurons as depth increases. This may be due to the increase in learning capacity of the deeper networks, as more hierarchical representations allow for the network to learn increasingly complex shapes compared to the shallower networks. Further, deeper networks have stronger long range connections due to a larger effective receptive field potentially resulting in

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{wraptable}{r}{7.4cm}
\def\arraystretch{1.15}
    %\vspace{-0.4cm}
     \centering
     \caption{Comparing dimensionality estimations for the \textit{texture} factor between two 
     methods. Both methods show that more texture neurons are found in
  representations with smaller receptive fields.}
     \vspace{-0.25cm}
 \resizebox{0.52\textwidth}{!}{
  \begin{tabular}{lcccccc}
  \specialrule{1.2pt}{1pt}{1pt}
    {\centering Method} &
    {\centering Res152} &
    {\centering Res101} &
    {\centering Res50} &
    {\centering Bag33} &
    {\centering Bag17} &
    {\centering Bag9} \\
    % \midrule
    \specialrule{1.2pt}{1pt}{1pt}
    \textbf{Net. Diss.} &
    433 &
    481 &
    499 &
    592 &
    623 &
    537 \\
    %\hline
    \textbf{Dim. est.} &
    661 &
    667 &
    692 &
    825 &
    839 &
    841 \\
    \specialrule{1.2pt}{1pt}{1pt}
    % Dim. est (Shape) & 371 & 365 & 349 & 284 & 278 & 276\\
  \end{tabular}}
  \label{tab:comparedissection}
  \vspace{-0.3cm}
\end{wraptable}
%%%%%%%%%%%%%%%%%%%%%%%%

%Finally, we assess the consistency between the dimensionality estimation
%technique and network dissection~\citep{bau2017network}, another method which
%estimates the number of neurons representing different concepts (described in
%Sec.~\ref{supp:consistency}). Because the latter cannot estimate shape
%dimensionalities, the comparison is limited to the texture dimensions shown in
%Table~\ref{tab:comparedissection}. Both methods predict a negative correlation
%between texture dimensionality and receptive field, except for BagNet9. The
%predicted absolute numbers differ due to two main reasons: First, both
%approaches rely on hyperparameters such as the baseline score and the IoU
%threshold.  Second, the semantic meaning of texture depends on the data, i.e.
%dimensionality estimation relies on the image pairs of SVOC and network
%dissection on the texture images in their dataset.  This might also explain the
%drop in detectors for BagNet9 if its receptive field is too small for some of
%the textures.  While absolute numbers depend on hyperparameters, results
%obtained with both methods are comparable across networks.
additional shape encoding neurons. The increase in shape understanding could be one of the reasons why deeper networks achieve better performance on various tasks, e.g., image classification. Finally, we assess the consistency between the dimensionality estimation
technique and network dissection~\citep{bau2017network}, another method which
estimates the number of neurons representing different concepts (described in
Sec.~\ref{supp:consistency}). Since network dissection cannot estimate shape
dimensionalities, the comparison is limited to the texture dimensions shown in
Table~\ref{tab:comparedissection}. Except for the case of BagNet9 and a
difference in the absolute numbers of neurons (discussed in
Sec.~\ref{supp:consistency}), both methods agree about the correlation between
texture dimensionality and the receptive field, which provides further evidence
that dimensionality estimates quantify the relevance of semantic
concepts faithfully.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]
% \def\arraystretch{1.15}
% \centering
% \caption{Dimensionality estimation of factors $|z_k|$ representing different semantic concepts for different networks.}
%      \vspace{-0.3cm}
% \resizebox{0.36\textwidth}{!}{

% 	\begin{tabular}{c|cc }

% 	\specialrule{1.2pt}{1pt}{1pt}
	 
% 	 \multirow{2}{*}{ \rotatebox{0}{Model}}  & \multicolumn{2}{c}{Factor $|z_k|$}\\
	 
% 	 \cline{2-3}
% 	   &  Shape & Texture\\
% 	 \specialrule{1.2pt}{1pt}{1pt}
	 
% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{AlexNet}}  &
	  

% 	  17.8\% & \textbf{31.7\%} \\
	  
% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{GoogleNet}}  &
	  

% 	  18.2\% & \textbf{31.6\%} \\
	  

% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{VGG-16}}  &
	  

% 	  17.3\% & \textbf{32.3\%}\\
	  
% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{SAN19-Patch}}  &
	  

% 	  18.8\% & \textbf{29.8\%}\\
	  
% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{SAN19-Pair}}  &
	  

% 	  14.9\% & \textbf{37.3\%}\\
	 
% 	\specialrule{1.2pt}{1pt}{1pt}

% 	\end{tabular}
	
% 	}

% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]
% \def\arraystretch{1.15}
% \centering
% \caption{Percentage of neurons ($|z_k|/|z|$) encoding different semantic concepts, $k$, for different stages of ResNet50 trained for various levels of shape bias. While a moderate percentage of neurons encode shape in stages $f_2$ and $f_3$, the majority of shape neurons are found in stage $f_5$, and networks with shape bias learn additional shape information in stage $f_5$.}
%      \vspace{-0.2cm}
% \resizebox{0.60\textwidth}{!}{

% 	\begin{tabular}{c|cc| cc | cc }

% 	\specialrule{1.2pt}{1pt}{1pt}
	
% 	 \multirow{3}{*}{\rotatebox{0}{Stage}} & \multicolumn{2}{c|}{\textbf{IN}} & \multicolumn{2}{c|}{\textbf{SIN}} & 
% 	 \multicolumn{2}{c}{\textbf{(SIN+IN)$\rightarrow$IN}}\\
% 	 \cline{2-7}
% 	  & \multicolumn{2}{c|}{Factor $|z_k|/|z|$} & \multicolumn{2}{c|}{Factor $|z_k|/|z|$} & \multicolumn{2}{c}{Factor $|z_k|/|z|$}\\
	  
% 	   \cline{2-7}
	 
% 	   &  Shape & Texture  &  Shape & Texture  &  Shape & Texture\\
% 	 \specialrule{1.2pt}{1pt}{1pt}
	 
% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{$f_2$}}  &
	  

% 	  14.1\% & \textbf{40.2\%} & 14.1\% & 40.6\% & 14.1\% & 40.6\% \\
	  
% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{$f_3$}}  &
	  

% 	  14.6\% & \textbf{39.5\%} & 14.8\% & 39.5\% & 14.8\% & 39.5\% \\
	  

% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{$f_4$}}  &
	  

% 	  15.3\% & \textbf{37.9\%} & 17.7\% & 34.7\% & 17.7\% & 34.8\% \\
	  
% 	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{$f_5$}}  &
	  

% 	  17.0\% & \textbf{33.8\%} & \textbf{26.2\%} & 23.3\% & 18.4\% & \textbf{31.2\%} \\
	  
	 
% 	\specialrule{1.2pt}{1pt}{1pt}

% 	\end{tabular}
	
% 	}

%     \label{tab:stage_wise_dim}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






% \begin{wrapfigure}{r}{0.5\textwidth}
%   \begin{center}
%   %\resizebox{1.0\textwidth}{!}{
%   \vspace{-0.22cm}
%       \includegraphics[width=0.48\textwidth]{figures/intro.eps} 
%   \end{center}
%   \vspace{-0.35cm}
% \caption{An illustration of how CNNs use position information to resolve boundary effects. We place CIFAR-10 images in random locations on a canvas of $0$'s (black) or $1$'s (white). We evaluate if a ResNet-18, trained w/ or w/o padding for semantic segmentation, can segment the image region. Surprisingly, performance is improved when either zero padding or a black canvas is used, implying position information can be exploited from border heuristics to reduce the boundary effect. Colormap is `viridis'; yellow is high confidence.}
%   \label{fig:intro}
%   \vspace{-0.45cm}
% \end{wrapfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{figure} [t]
%   \begin{center}
%   \resizebox{0.50\textwidth}{!}{ 
%   %\vspace{-0.55cm}
%       \includegraphics[width=0.50\textwidth]{figures/shape.pdf}}
%   \end{center}
%   % \vspace{-0.35cm}
%   \caption{Sample generation of validation examples for different semantic concepts.}
%   \label{fig:stylize}
%   %\vspace{-0.45cm}
% \end{figure}
%\vspace{-0.2cm}
% \subsubsection{Stage-Wise Analysis of Shape and Texture Dimensionality}\label{sec:dim_stage}

\textbf{Stage-Wise Analysis of Shape and Texture Dimensionality}
We now explore \textit{where} CNNs encode shape by applying the
dimensionality estimation method with the latent representations from ResNet50 stages one to five with different amounts of shape bias. Due to the different dimensions 
%%%%%%%%%%%%%%%%%%%%%
\begin{wraptable}{r}{8.9cm}
\def\arraystretch{1.15}

     \vspace{-0.2cm}
     \centering
    \caption{Percentage of neurons ($|z_k|/|z|$) encoding different semantic concepts, $k$, for different stages of ResNet50 trained for various levels of shape bias. While a moderate percentage of neurons encode shape in stages $f_1$, $f_2$, and $f_3$, the majority of shape neurons are found in stage $f_5$. Networks with shape bias learn additional shape information in stage $f_5$.}
     \vspace{-0.2cm}
\resizebox{0.62\textwidth}{!}{

	\begin{tabular}{c|cc| cc | cc }

	\specialrule{1.2pt}{1pt}{1pt}
	
	 \multirow{3}{*}{\rotatebox{0}{Stage}} & \multicolumn{2}{c|}{\textbf{IN}} & \multicolumn{2}{c|}{\textbf{SIN}} & 
	 \multicolumn{2}{c}{\textbf{(SIN+IN)$\rightarrow$IN}}\\
	 \cline{2-7}
	  & \multicolumn{2}{c|}{Factor $|z_k|/|z|$} & \multicolumn{2}{c|}{Factor $|z_k|/|z|$} & \multicolumn{2}{c}{Factor $|z_k|/|z|$}\\
	  
	   \cline{2-7}
	 
	   &  Shape & Texture  &  Shape & Texture  &  Shape & Texture\\
	 \specialrule{1.2pt}{1pt}{1pt}
	 
	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{$f_1$}}  &
	  

	  12.5\% & 42.2\% & 12.5\% & 42.2\% & 12.5\% & 42.2\% \\
	  
	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{$f_2$}}  &
	  

	  14.1\% & 40.2\% & 14.1\% & 40.6\% & 14.1\% & 40.6\% \\
	  
	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{$f_3$}}  &
	  

	  14.6\% & 39.5\% & 14.8\% & 39.5\% & 14.8\% & 39.5\% \\
	  

	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{$f_4$}}  &
	  

	  15.3\% & 37.9\% & 17.7\% & 34.7\% & 17.7\% & 34.8\% \\
	  
	  \multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{$f_5$}}  &
	  

	  17.0\% & 33.8\% & 26.2\% & 23.3\% & 18.4\% & 31.2\% \\
	  
	 
	\specialrule{1.2pt}{1pt}{1pt}

	\end{tabular}
	
	}

    \label{tab:stage_wise_dim}
%\vspace{-0.3cm}
\end{wraptable} 
%%%%%%%%%%%%%%%%%%%%%%%%
at each of these stages, we present the results as the
percentage of dimensions encoding the particular semantic factor, $|z_k|/|z|$, where $|z|$ refers to length of the latent representation.
Table~\ref{tab:stage_wise_dim} shows that \textit{all stages of the network} encode shape with an increase in the last two stages. Further, biasing the models towards shape only changes the percentage of shape encoding in the final two stages. Beginning at the fourth stage, there is a significant jump in the number of shape
dimensions for all three models with the shape biased models having a larger increase. At the final stage, latent
representations encode even more shape, where SIN in particular has a large increase of 8.5\%. This indicates that biasing a model towards shape mainly affects the last two stages of the network, suggesting that future
work could focus on improving the shape bias of earlier layers.
An increase in shape dimensions is \textit{inversely
proportional} to the amount of texture dimensions. Notably, from
stage four to stage five, there is a large drop in the amount of texture
dimensions for all networks.
%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsubsection{When Does Shape Become Relevant During ImageNet Training?}\label{sec:dim_training}
\textbf{When Does Shape Become Relevant During Training?}
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{wrapfigure}{r}{0.7\textwidth}
%   \begin{center}
%   %\resizebox{1.0\textwidth}{!}{
%   \vspace{-0.65cm}
%         \resizebox{0.7\textwidth}{!}{ 
%   %\vspace{-0.55cm}
%       \includegraphics[width=0.48\textwidth]{figures/dim_s4.pdf} \hspace{0.2cm}
%       \includegraphics[width=0.48\textwidth]{figures/dim.pdf}
%     %   \hspace{0.3cm}
%     %   \includegraphics[width=0.48\textwidth]{figures/dim_stage3.pdf}
%       }
%   \end{center}
%   \vspace{-0.4cm}
% \caption{Analyzing the number of dimensions in a ResNet50 which encode shape ($|z_{shape}|$) and texture ($|z_{texture}|$) over the course of ImageNet training. Dimensions are estimated using stage four (Left, $|z^{(4)}|=1024$) and stage five (Right, $|z^{(5)}|=2048$) latent representations. When training begins, $z$ is very sensitive to \textit{texture} and over the course of training learns to focus on the \textit{shape} instead. Surprisingly, the number of shape encoding neurons increases in only the first 25 epochs, and then saturates thereafter. The vertical lines represent multiplying the learning rate by a factor of 0.1.}
%   \label{fig:epoch}
%   \vspace{-0.45cm}
% \end{wrapfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In this section we aim to semantically understand \textit{how} a network learns to solve the ImageNet classification problem by focusing on the relevant semantic information (e.g., \textit{shape} and \textit{texture}) while discarding task-irrelevant information (e.g., color). 
\textcolor{black}{To answer the question `When do models learn to encode shape and texture during training?', we capture the changes of \textit{shape} and \textit{texture} occurring over the course of training a classifier on ImageNet (IN) and Stylized ImageNet (SIN). We obtain 18 different instances of a ResNet50 model during training on IN and SIN, each representing a checkpoint between epochs 0 and 90 (equally distributed). For each checkpoint, we measure the dimensionality of shape and texture semantic factors and plot the results in Fig.~\ref{fig:epoch}. The shape factor in the stage-5 latent representations for both IN (Fig.~\ref{fig:epoch} middle) and SIN (Fig.~\ref{fig:epoch} right) models become increasingly more relevant during the course of training, however the percentage of dimensions grows much larger and faster in the case of the SIN trained model. The texture factor decreases as the training progresses in both cases as well. For the stage-4 representation in a model trained on IN (Fig.~\ref{fig:epoch} left), note that the shape encoding neurons increase only marginally over the course of training. This further reveals that a large proportion of shape information is encoded at the deepest layer.} 


% We see that the \textit{shape} factor becomes increasingly more relevant when we use the latent dimension from stage-5 (Fig.~\ref{fig:epoch} (right)), while the texture factor decreases as the training progresses. In the case of the stage-4 latent representation (Fig.~\ref{fig:epoch} (left)), the dimensionality of shape encoding does not increase as training progresses. This further reveals that a large proportion of shape information is encoded at the deepest layer.}
%Further, we showed that the shape information is largely contained in the last few layers of a CNN (i.e., stage four and five of a ResNet)We now explore \textit{when} a CNN becomes biased towards texture during training and in parallel seek to find out when shape information is learned. 
%- say how shape encoding of early layers does not change over training
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\vspace{-0.3cm}
\centering
  \begin{center}
  \resizebox{0.99\textwidth}{!}{ 
  \vspace{0.2cm}
      \includegraphics[width=0.33\textwidth, height=3.65cm]{figures/dim_stage4.pdf} \hspace{0.1cm}
      \includegraphics[width=0.33\textwidth]{figures/dim_stage5.pdf} 
      \hspace{0.1cm}
      \includegraphics[width=0.33\textwidth]{figures/SIN_dim_stage5.pdf}

      }
  \end{center}
  \vspace{-0.35cm}
  \caption{\textcolor{black}{Analyzing the number of dimensions in a ResNet50 which 
  encode shape ($|z_{shape}|$) and texture ($|z_{texture}|$) over the course of ImageNet (IN, left two) and Stylized ImageNet (SIN, right) training. Dimensions are estimated using stage four, $|z^{(4)}|=1024$, and stage five, $|z^{(5)}|=2048$, latent representations. When training begins, $z$ is very sensitive to \textit{texture} but over the course of training learns to focus on the \textit{shape} instead (faster in SIN case). The vertical lines represent multiplying the learning rate by a factor of 0.1. Note that the estimated dimensions differ slightly from Table~\ref{tab:table1} as we trained the IN and SIN models used in this figure from scratch.}}
  \label{fig:epoch}
  \vspace{-0.4cm}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.2cm}
\section{How Much Shape Information do CNNs Encode?}\label{sec:how_much_shape}
\textcolor{black}{The previous section measured the dimensionality of shape encodings for various CNNs and settings. We now aim to evaluate the quality of these encodings, and whether more shape encoding neurons implies that more robust shape information can be extracted from these latent representations. We also conduct a set of experiments by targeting the shape and texture-specific neurons (see Sec~\ref{sec:remove_target} for results and discussion), revealing an additional link between the two techniques used in our paper (i.e., dimensionality estimation and read-out module).
% We now aim to see if the number of neurons used to encode shape implies that more robust boundary and semantic information can be extracted from these latent representations.
~\cite{hermann2019exploring} measured the quality of shape encodings in a CNN's latent representations by training a linear classifier on the CNN's late-stage features to predict the shape label of SIN images. Quantifying shape information by using image level labels does not allow for the per-pixel evaluation of the encoded shape, and its relation to the associated categorical label, two key components for fully evaluating the shape information contained in a particular encoding.}

% it prevents the separate analysis of shape (i.e., class-agnostic silhouette) and semantics (i.e., semantic silhouette), as `shape bias' is, by definition, the classification accuracy. Second, it does not allow for a spatial (i.e., pixel-level) evaluation to be performed, a key component for fully evaluating the shape information contained in a particular encoding.

% First, it prevents the separate analysis of shape (i.e., class-agnostic silhouette) and semantics (i.e., semantic silhouette), as `shape bias' is, by definition, the classification accuracy. Second, it does not allow for a spatial (i.e., pixel-level) evaluation to be performed, a key component for fully evaluating the shape information contained in a particular encoding.

% has three main drawbacks: (i) the linear classifier may be able to predict the shape label without using the entire object shape (e.g., recognizing a `bicycle' looking solely at the wheel spokes), (ii) quantifying shape via the semantic label does not allow for the separate analysis of shape and semantics, and (iii) image level classification fails to spatially quantify the amount of shape information (i.e., \textit{where} in the image is the shape captured?).

\subsection{Quantifying Shape Information in CNN Latent Representations}
To overcome the aforementioned issues, we consider two tasks which require a detailed understanding of object shape: \textit{binary} and \textit{semantic} segmentation. A `shape encoding network' (SEN), the network being analyzed, consists of a CNN with fixed weights. We then train a shallow read-out module that takes a latent representation from the SEN, to predict a segmentation map (i.e., binary or semantic). If the read-out module can accurately segment objects with \textit{a binary mask}, we conclude the SEN encodes the precise shape of the objects of interest. Further, the read-out modules ability to perform \textit{semantic} segmentation, measures how much of this encoded shape is successfully localized with per-pixel categorical information. We use ResNet networks of various depths (i.e., 34, 50, and 101) as SENs with a readout module containing either one or three convolution layers with 3$\times$3 kernels. We use the \textit{trainaug} and \textit{val} split of the VOC 2012 dataset to train and test the read-out module, respectively. The binary segmentation ground truth labels are generated by converting all semantic categories to a single `object' class. \textcolor{black}{Note that the binary segmentation and semantic segmentation experiments are done completely independently of one another}.
% This distinction enables us to \textit{disentangle} the networks understanding of \textit{shape} and \textit{semantic} information as the network may understand the shape of the object without being able to predict the semantic class, and vice-versa. 

%%%%%%%%%%%%%%%%%%%%%
\begin{table}[b]
\vspace{-0.2cm}
\def\arraystretch{1.1}
\centering
\caption{\textbf{Left:} We measure the amount of shape encoded in frozen CNN by training a read-out module on either binary (\textit{Bin}) or semantic  segmentation (\textit{Sem}) under different training settings. `None': random initialization, `End-to-End': network is not frozen and trained with the read-out module, `IN': pre-trained on ImageNet. \textbf{Right:} Shape information contained in various shape biased models.} % IF LOOKING FOR SPACE, MAYBE IT'S NOT NECESSARY TO REPEAT WHAT IN, SIN, SIN+IN->IN ARE HERE?
     \vspace{-0.2cm}
\resizebox{1.0\textwidth}{!}{
	\begin{tabular}{c||cc|cc|cc||cc|cc|cc }
	\specialrule{1.2pt}{1pt}{1pt}
	 
	 \multirow{3}{*}{\hspace{0.01cm} \rotatebox{0}{Training}} 
	 &\multicolumn{6}{c||}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{1 Layer Readout}} }  &\multicolumn{6}{c}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{3 Layers Readout}} }\\
	 
	 \cline{2-13}
	 
	 &\multicolumn{2}{c|}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{ResNet34}}} }
	 &\multicolumn{2}{c|}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{ResNet50}}} } &\multicolumn{2}{c||}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{ResNet101}}} } 
	 &\multicolumn{2}{c|}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{ResNet34}}} }
	 &\multicolumn{2}{c|}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{ResNet50}}} } &\multicolumn{2}{c}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{ResNet101}}} }   \\
	
	 \cline{2-13}
	 &\textit{Bin} & \textit{Sem} &\textit{Bin} & \textit{Sem} &\textit{Bin} & \textit{Sem} & \textit{Bin} & \textit{Sem}
	 & \textit{Bin} & \textit{Sem}
	 &\textit{Bin} & \textit{Sem}\\
				
	\specialrule{1.2pt}{1pt}{1pt}
	
	None & 46.5 &5.2&48.0&6.1 &44.9&5.1 &58.0 & 7.2 & 58.0 & 6.0 & 55.0 & 4.8 \\
	End-to-End & 80.2 &63.4& 80.2 &62.7& 81.0 &65.8& 82.1 & 67.7 & 82.2 & 68.1 & 82.9 & 71.5 \\
	IN & 66.3 &48.1& 70.6 &50.9& 72.1 &51.9& 78.9 & 59.1 & 79.8 & 61.6 & 80.4 & 63.4 \\
	
	\specialrule{1.2pt}{1pt}{1pt}
	\end{tabular}
	\hspace{0.1cm}
	\begin{tabular}{c|cc }
	\specialrule{1.2pt}{1pt}{1pt}
	 
	 \multirow{2}{*}{\hspace{0.01cm} \rotatebox{0}{Training}} 
	 &\multicolumn{2}{c}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{ResNet50}}} }
  \\
	\cline{2-3}
	 & \textit{Bin} & \textit{Sem}\\
				
	\specialrule{1.2pt}{1pt}{1pt}
	
% 	IN$\rightarrow$VOC &  70.6 & 50.9 \\
% 	IN$\rightarrow$SVOC &  58.7 & 21.8  \\
% 	SIN$\rightarrow$VOC &  67.2 & 42.6 \\
	
% 	SIN$\rightarrow$SVOC &  62.1 & 31.1 \\
	
	IN &  79.8 & 61.6 \\
	SIN &  76.4 & 53.7 \\
	
	(SIN+IN)$\rightarrow$IN&  77.8 & 58.0\\
	
	\specialrule{1.2pt}{1pt}{1pt}
	\end{tabular}
	
	}
    \label{tab:readout_1}
    \vspace{-0.3cm}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Results}\label{sec:readout_results}
Table~\ref{tab:readout_1} presents the results in terms of mean-Intersection-over-Union (mIoU) under different initialization settings with; `IN': a SEN trained for ImageNet classification, `None': a SEN with random weight initialization and without any training, `End-to-End': the SEN and readout module trained in an end-to-end manner on either the binary (\textit{Bin}) or semantic (\textit{Sem}) segmentation ground truth. The None and End-to-End networks represent lower and upper bounds for encoding shape, respectively. All read-out modules in this section are trained on the last layer's latent representations. Interestingly, three convolutional layers can extract similar amounts of shape information from the IN-SEN as the End-to-End-SEN. For example, training the ResNet101 End-to-End-SEN for \textit{Bin} improves the mIoU by merely 2.5\% compared to the IN-SEN. ImageNet trained CNNs also contain shape encodings which successfully localize per-pixel categorical information as well, which can be seen when comparing the performance of the IN-SEN and End-to-End SEN, e.g., for ResNet50, the IN-SEN and  End-to-End-SEN achieve 61.6\% and 68.1\%, respectively. This is an interesting result considering the difficulty of semantic segmentation and that \textit{none} of the IN-SEN weights are trained for pixel-wise objectives. Shape information also increases relative to the depth of the network which supports the results presented in Table~\ref{tab:table1}(c). As expected, the End-to-End-SEN and IN-SEN contain significantly more shape information in their latent representations than the baseline None-SEN.

We now evaluate the shape information encoded in networks which have different levels of shape bias. We compare the \textit{Bin} and \textit{Sem} performance of the read-out module trained on the features of three different SENs trained on IN, SIN, and (SIN+IN)$\rightarrow$IN. As the validation is on non-stylized images, SIN-SEN has slightly lower performance for \textit{Bin}, and significantly less performance on \textit{Sem}. Such a large difference in performance implies that while the boundary of the object is known, it is difficult for the network to correctly assign per-pixel \textit{categorical} information, a phenomenon further explored in Sec.~\ref{sec:does_shape}. Interestingly, the (SIN+IN)$\rightarrow$IN-SEN also has slightly lower performance than the IN-SEN for \textit{Bin}, but does not suffer in performance as much as the SIN-SEN in the case of \textit{Sem}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Where is Shape Information Stored?}\label{sec:where_shape}

\textbf{Where is Shape Information Stored?}
\begin{table}[t]
\vspace{-0.3cm}
	\centering
	\begin{minipage}{0.40\linewidth}
	\caption{Shape encoding results for different stages of ResNet networks trained on ImageNet. Combining features from early stages increases shape encoding.} 
	\centering
	\vspace{-0.2cm}
	\def\arraystretch{1.1}
	\setlength\tabcolsep{3.2pt}
		\resizebox{0.99\textwidth}{!}{
			\begin{tabular}{ccccc|cc|cc }
	\specialrule{1.2pt}{1pt}{1pt}
	\multirow{2}{*}{\hspace{0.01cm} \rotatebox{0}{$f_1$}} &
	  \multirow{2}{*}{\hspace{0.01cm} \rotatebox{0}{$f_2$}} & \multirow{2}{*}{\hspace{0.01cm} \rotatebox{0}{$f_3$}} & \multirow{2}{*}{\hspace{0.01cm} \rotatebox{0}{$f_4$}}  &\multirow{2}{*}{\hspace{0.01cm} \rotatebox{0}{$f_5$}} &\multicolumn{2}{c|}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{ResNet50}}} } &\multicolumn{2}{c}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{ResNet101}}} }   \\
	\cline{6-9}
	&&&& &\textit{Bin} & \textit{Sem} & \textit{Bin} & \textit{Sem}\\
	\specialrule{1.2pt}{1pt}{1pt}
	$\checkmark$ &&&&& 44.7& 4.6& 42.3& 4.7\\
	&$\checkmark$ &&&& 52.7& 6.4& 53.0& 5.6\\
	&&$\checkmark$&&& 59.6 &10.9 & 57.7&9.4\\
	&&&$\checkmark$&& 70.8 & 33.9 & \textbf{73.2}&43.6\\
	 &&&&$\checkmark$& \textbf{70.6} & \textbf{50.9} & 72.1&\textbf{51.9}\\
	 \midrule
	 &$\checkmark$ & $\checkmark$&&& 66.0 & 16.6 & 63.8&13.5\\
	  &$\checkmark$ & $\checkmark$& $\checkmark$&& 74.5 & 42.2 &76.8&49.8 \\
	 &$\checkmark$&$\checkmark$&$\checkmark$ &$\checkmark$ & \textbf{77.3} & \textbf{53.7} & \textbf{78.2}& \textbf{56.2}\\
	 
	 $\checkmark$ &$\checkmark$&$\checkmark$&$\checkmark$ &$\checkmark$ & \textbf{77.3}& 52.9& \textbf{78.2} & 55.2 \\

	\specialrule{1.2pt}{1pt}{1pt}
	\end{tabular}\label{tab:stage_readout}
			}
	\end{minipage} \hfill   
	\begin{minipage}{0.59\linewidth}
	      %\vspace{0.7cm}
          \centering
         \resizebox{0.99\textwidth}{!}{
          \includegraphics[width=0.59\textwidth]{figures/seg_stage_new.pdf} 
    }
  \vspace{-0.27cm}
  \captionof{figure}{Stage-wise predictions of read-out module on binary (\textit{Bin}) and semantic (\textit{Sem}) segmentation.}
  \label{fig:seg_stage}
	\end{minipage} 
	    
	\vspace{-0.5cm}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%
We now examine if the large amount of \textit{shape} information contained in ImageNet pretrained models is equally distributed across different stages of the CNN. 
\begin{wrapfigure}{r}{0.430\textwidth}
  \begin{center}
  %\resizebox{1.0\textwidth}{!}{
  \vspace{-0.38cm}
      \includegraphics[width=0.4\textwidth]{figures/shape_seg.pdf} 
  \end{center}
  \vspace{-0.35cm}
  \caption{Quantifying the shape and semantic information encoded by a CNN over the course of ImageNet training. A separate read-out module is trained on the frozen CNN weights for each snapshot. Vertical lines represent the learning rate decay.}
  \label{fig:readout_imagenet_training}
  \vspace{-0.4cm}
\end{wrapfigure}
In this experiment, we train read-out modules on features from different stages, ($f_1, f_2, f_3, f_4, f_5$), of the SEN to examine which stage of a CNN encodes shape information. Note that we only use one layer readout modules for this experiment. As shown in Table~\ref{tab:stage_readout}, the read-out module trained on the last stage features, ($f_4, f_5$), achieves higher performance compared to the earlier stage features, ($f_1, f_2, f_3$), for both \textit{Bin} and \textit{Sem}. This is to be expected, as feature maps from later stages have higher channel dimensions and larger effective receptive fields compared to the feature maps extracted from earlier layers. A surprising amount of shape information (i.e., \textit{Bin}) can be extracted from stages $f_1, f_2$ and $f_3$; however, these features lack high-level \textit{semantics} to correlate with this shape information,
\textcolor{black}{which can be observed as the corresponding \textit{Sem} performance is much lower. Figure~\ref{fig:seg_stage} reveals this phenomenon; the \textit{horse} and \textit{person} are outlined even for the early stage binary masks, but are only labelled with correct per-pixel categorical assignments in the later stages. Considering the non-trivial amount of shape information contained in the early stages, we investigate if aggregating multi-stage features encodes more shape compared to the last stage feature, ($f_5$). Table~\ref{tab:stage_readout} (bottom) shows that training a readout module on multi-stage features significantly improves the \textit{Bin} and \textit{Sem} performance, suggesting that tasks requiring shape information may benefit from hypercolumn style architectures~\citep{hariharan2015hypercolumns}. This indicates that some \textit{shape} information is encoded in earlier layers but not captured in the late stages, which agrees with the dimensionality estimation results in Table~\ref{tab:stage_wise_dim}, as around 12.5\% and 14\% of neurons encode shape in the first stage and second stage, respectively.}
% DOES THIS IMPLY THAT A HYPERCOLUMN STYLE READOUT WOULD BE USEFUL FOR TASKS REQUIRING SHAPE INFORMATION? MAYBE WE MENTION THIS IF SO?
%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{When do CNNs Encode Shape During ImageNet Training?}\label{sec:read_when}
\textbf{When do CNNs Encode Shape During ImageNet Training?}
%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%
Now we quantify the amount of shape encoded in the latent representations over
the same ImageNet training snapshots as in Sec.~\ref{sec:dimension}.
Fig.~\ref{fig:readout_imagenet_training} shows the performance of the read-out
module trained on the frozen SEN every five epochs, as well as the ResNet50's validation accuracy on ImageNet classification.
Note that we train a separate read-out module for every snapshot. Similar to the findings in Fig.~\ref{fig:epoch}, we see that the majority of both binary and semantic shape information is learned within the first 10 epochs i.e., $\frac{77.1\%}{79.4\%} = 97.1\%$ of the final \textit{Bin} mIoU and
$\frac{52.9\%}{60.0\%} = 88.2\%$ of the final \textit{Sem} mIoU is
obtained by the read-out module after only 10 epochs. 
% This agrees with the findings from Fig.~\ref{fig:epoch} where the majority of shape encoding dimensions are learned within 20 epochs. 
Contrasting purely shape
related information (i.e., \textit{Bin}), a small but significant
portion of \textit{per-pixel categorical} information is learned after the initial 10 epochs, when the learning rate decay is employed. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table} [t]
%\vspace{-0.2cm}
	\centering
	\begin{minipage}{0.29\linewidth}
	\caption{Shape encoding results for shape biased ResNet50s on \textit{stylized} VOC12 validation set.} %and evaluated on two different GT patterns
	\centering
	\vspace{-0.3cm}
	\def\arraystretch{1.1}
	\setlength\tabcolsep{3.2pt}
		\resizebox{0.95\textwidth}{!}{
			\begin{tabular}{c|cc }
	\specialrule{1.2pt}{1pt}{1pt}
	 
	 \multirow{2}{*}{\hspace{0.01cm} \rotatebox{0}{Training Data}} 
	 &\multicolumn{2}{c}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{ResNet50}}} }
  \\
	\cline{2-3}
	 &Bin. & Sem.\\
				
	\specialrule{1.2pt}{1pt}{1pt}
	
	IN &  45.7 & 8.5 \\
	SIN &  60.3 & 26.4 \\
	(SIN+IN)$\rightarrow$ IN&  44.5 & 9.0 \\
	
% 	IN &  57.3 & 22.2 \\
% 	SIN &  71.9 & 42.8 \\
% 	(SIN+IN)$\rightarrow$ IN&  58.3 & 23.1\\
	
	\specialrule{1.2pt}{1pt}{1pt}
	\end{tabular}\label{tab:readout_svoc}
			}
	\end{minipage} \hfill
	\begin{minipage}{0.68\linewidth}
	      %\vspace{0.7cm}
          \centering
         \resizebox{1.0\textwidth}{!}{
          \includegraphics[width=0.5\textwidth]{figures/seg_style_new.pdf} 
    }
  \vspace{-0.6cm}
      \captionof{figure}{Binary and semantic segmentation masks extracted from CNNs trained on ImageNet (\textbf{IN}) and Stylized ImageNet (\textbf{SIN}). }
%   Both networks encode the \textit{shape} (shown as heatmap) reasonably well, but fail to assign the correct categorical label to the objects of interest.
  \label{fig:seg_style}
	\end{minipage} 
	    
	\vspace{-0.35cm}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Does Knowing an Object's Shape Imply Knowing Its Semantic Class?}\label{sec:does_shape}
% \noindent \textbf{Does Knowing an Object's Shape Imply Knowing Its Semantic Category?}
The results in Secs.~\ref{sec:readout_results} and~\ref{sec:dimension} suggest that encoding the object \textit{shape} may not imply the network also captures the object \textit{class} on a per-pixel level. Table~\ref{tab:readout_1}(b) shows that shape biased models lose their ability to relate \textit{categorical} activations to localized object regions. The stage-wise results from Table~\ref{tab:stage_readout} further demonstrate that a modest amount of shape information is contained in early stage features but that categorical information can only be correctly assigned to pixels at the last two stages, which can also be seen in Fig.~\ref{fig:seg_stage}. To further test this hypothesis, we validate various SENs and their read-out modules on stylized VOC12 \textit{val} images rather than non-stylized images. Note that the val images are stylized by a single randomly selected texture from the same set of textures used in Sec.~\ref{sec:dimension}. This ensures that the networks must rely solely on the object's shape rather than the texture to make predictions. The \textit{difference} in performance between the \textit{Bin} mIoU and \textit{Sem} mIoU can therefore approximate the amount of shape information that is \textit{not} correlated to its corresponding \textit{semantic} class. As shown in Table~\ref{tab:readout_svoc}, the large difference in performance between \textit{Bin} and \textit{Sem} suggests that these SENs capture the shape of the object but lack the ability to correctly assign per-pixel semantic labels to these objects, even in the last layer of the network. Qualitative results are presented in Fig.~\ref{fig:seg_style}; note how the binary mask (presented as likelihood heatmaps) for the SIN trained model reasonably segments the objects, while the semantic masks fail to resemble realistic predictions, i.e., \textit{multiple} object categories are placed spuriously over and around the object of interest. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{Does Learning Semantics Increases Shape Encoding?} 
% While intuition might suggest that shape information encoded at higher layer are shared by high-level semantics, it is natural to analyze if learning for per pixel semantic objective increases shape encoding in CNNs. To answer this question, we estimate the dimensionality of shape factor trained for different semantic objectives (e.g., image classification, binary segmentation, and semantic segmentation). Table presents the dimensionality estimation results of different semantic factors. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.2cm}
\subsection{Targeting and Removing Shape and Texture Neurons} \label{sec:remove_target}
In Sec.~\ref{sec:docnns}, we used a dimensionality estimation technique to estimate the number of dimensions which encode shape and texture in a CNNs latent representations. Given these neurons, we now validate if the most shape specific, or texture specific, neurons can influence the performance of a read-out module when removing these specific neurons during inference. We hypothesize that the network trained on Stylized ImageNet (i.e., a \textit{shape biased model}) will be more reliant on the shape neurons than a network trained on ImageNet (i.e., a \textit{texture biased model}) which are known to naturally exhibit a texture bias. See Appendix~\ref{sec:keep_target} for additional experiments where we keep solely the targeted neurons instead of remove them. To asses this hypothesis, we conduct a series of read-out module experiment and invoke the same settings as Sec.~\ref{sec:how_much_shape} are imposed. However, during this experiment we manipulate the latent representation as an image passes through the ResNet-50, before it is fed through the read-out module. More specifically, we rank the neurons by mutual information for both the \textit{shape} and \textit{texture} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{wraptable}{r}{8.0cm}
% \begin{table}[t]
	\centering
	\caption{Shape encoding results for ResNet50's trained on ImageNet (IN) and stylized ImageNet (SIN) based read-out modules when the top $N$ \textit{shape} or \textit{texture}-specific neurons are removed from the latent representation during inference. Removing the top $N$ shape specific neurons from the SIN-read-out hurts the network's shape-recognition abilities more compared to the IN-read-out model.} 
	\centering
	\def\arraystretch{1.3}
	\setlength\tabcolsep{3.7pt}
		\resizebox{0.58\textwidth}{!}{
			\begin{tabular}{c|cccc|cccc|cccc }
	\specialrule{1.2pt}{1pt}{1pt}
	
		\multirow{3}{*}{\hspace{0.01cm} \rotatebox{0}{$N$}}  & \multicolumn{4}{c|}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{Shape}} } & \multicolumn{4}{c|}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{Texture}} } & \multicolumn{4}{c}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{Residual}} }\\
 \cline{2-13}
 
 &\multicolumn{2}{c}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{IN}}} } &\multicolumn{2}{c|}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{SIN}}} } &\multicolumn{2}{c}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{IN}}} } &\multicolumn{2}{c|}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{SIN}}} } 
 &\multicolumn{2}{c}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{IN}}} } &\multicolumn{2}{c}{\multirow{1}{*}{\hspace{0.01cm} \rotatebox{0}{\textbf{SIN}}} } \\
	 \cline{2-13}
	 
	 &\textit{Bin} & \textit{Sem} & \textit{Bin} & \textit{Sem} &\textit{Bin} & \textit{Sem} & \textit{Bin} & \textit{Sem} &\textit{Bin} & \textit{Sem} & \textit{Bin} & \textit{Sem}\\
	\specialrule{1.2pt}{1pt}{1pt}
	
	\textbf{0} & \textbf{70.6} & \textbf{50.9} & \textbf{76.4} & \textbf{53.7}& \textbf{70.6} & \textbf{50.9} & \textbf{76.4} & \textbf{53.7} & \textbf{70.6} & \textbf{50.9} & \textbf{76.4} & \textbf{53.7}\\
	\hline
	
	\textbf{100} & 68.8& 46.4 & 64.6& 37.1 & 69.3& 44.7 & 65.7& 39.2 & 68.3& 46.7 & 64.7& 37.3 \\
	
	\textbf{200} & 67.9 &40.0 & 57.3& 31.4 & 67.9& 39.7 & 62.5& 32.7 &66.1 &44.2 & 64.9& 34.8 \\
	
	\textbf{300} & 61.6& 38.0 & 58.6& 25.8 & 66.3& 37.6 & 55.0& 27.9& 62.9&40.0 & 62.3& 30.1\\
	
	
	\specialrule{1.2pt}{1pt}{1pt}
	\end{tabular}
			}
	\label{tab:neurons_remove}
	\vspace{-0.3cm}

\end{wraptable}
%%%%%%%%%%%%%%%%%%%
semantic factors, and then identify the top $N$ of neurons from either the shape or texture neurons. We then \textit{remove these neurons} before passing the latent representation to the read-out module by simply setting the features at these dimensions to zero. This allows us to identify which neurons in each network (i.e., the shape biased or texture biased model) are relied on more heavily to encode shape and semantic information. Note that for this experiment, no training occurs. The goal is to simply measure the difference in inference performance when removing $N$ shape-specific neurons, or $N$ texture-specific neurons. Therefore we simply take the trained models and read-out modules from Sec.~\ref{sec:how_much_shape} to perform inference while masking out the targeted neurons. Note that validation is done on the \textit{val} split from (non-stylized) VOC 2012. 
% \subsubsection{Results}
% Figures~\ref{fig:keep_neuron_target} and~\ref{fig:remove_neuron_target} illustrate the binary and semantic segmentation results in terms of mIoU obtained from training read-out modules on IN and SIN trained ResNet-50s, respectively (\textbf{Experiment 1}). It is clear that for the model biased towards texture (IN pretrained), keeping texture neurons while removing all other neurons results in a better performance than keeping only the shape neurons. In contrast, Fig.~\ref{fig:remove_neuron_target} shows that for shape-biased model (SIN pretrained), keeping shape-specific neurons achieves better performance than keeping only texture-specific neurons. These results support the hypothesis that the network trained on Stylized ImageNet (i.e., a shape biased model) is not only biased towards making predictions based on object shape, but more reliant on shape-specific neurons than a network trained on IN. 

\noindent \textbf{Results.} Table~\ref{tab:neurons_remove} presents the binary and semantic segmentation results in terms of mIoU. We report the results under three different settings; (i) top $N$ \textit{shape-specific} neurons removed, (ii) top $N$ \textit{texture-specific} neurons removed, and (iii) top $N$ \textit{residual} neurons removed. Note that for this experiment, we do not train the read-out module. Instead, we first remove the specified neurons, and then run inference using the pretrained IN and SIN models as well as the already trained read-out modules. Interestingly, we find that gradually removing the \textit{shape-specific} neurons from SIN pretrained model more significantly hurts performance than the IN pretrained model. For instance, removing 100 shape-specific neurons from SIN achieves 37.1\% \textit{sem} mIoU, while the performance dropped to 25.8\% \textit{sem} IoU when the top 300 shape-specific neurons are removed (i.e., an 11.3\% drop). When comparing this to the performance drop of the IN trained model, we see that the difference is lower, from 46.4\% to 38.0\% (i.e., an 8.4\% drop). This further supports the hypothesis that SIN trained models are more reliant on the individual shape encoding neurons than the texture encoding neurons. In addition, removing shape-specific neurons from SIN pretrained model hurts performance more than removing the texture neurons. For example, when removing 300 shape neurons for the SIN trained model, the performance drops to 25.8\%, while removing 300 texture-specific neurons decreases the performance to only 27.9\%. Finally, we observe that removing \textit{shape or texture} specific neurons hurts performance more than removing the residual neurons. This suggests that shape and texture are the two most important semantic factors for a network to encode and that other semantic factors contained in the residual (e.g., color, lighting) are not as discriminative for the task of image classification. 
